Problematic Machine Behavior: A Systematic Literature Review of Algorithm Audits

While algorithm audits are growing rapidly in commonality and public importance, relatively little scholarly work has gone toward synthesizing prior work and strategizing future research in the area. This systematic literature review aims to do just that, following PRISMA guidelines in a review of over 500 English articles that yielded 62 algorithm audit studies. The studies are synthesized and organized primarily by behavior (discrimination, distortion, exploitation, and misjudgement), with codes also provided for domain (e.g. search, vision, advertising, etc.), organization (e.g. Google, Facebook, Amazon, etc.), and audit method (e.g. sock puppet, direct scrape, crowdsourcing, etc.). The review shows how previous audit studies have exposed public-facing algorithms exhibiting problematic behavior, such as search algorithms culpable of distortion and advertising algorithms culpable of discrimination. Based on the studies reviewed, it also suggests some behaviors (e.g. discrimination on the basis of intersectional identities), domains (e.g. advertising algorithms), methods (e.g. code auditing), and organizations (e.g. Twitter, TikTok, LinkedIn) that call for future audit attention. The paper concludes by offering the common ingredients of successful audits, and discussing algorithm auditing in the context of broader research working toward algorithmic justice.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> acmart-preload-hook.tex <==
\PassOptionsToPackage{table}{xcolor}

==> cut.tex <==
\setlength{\tabcolsep}{10pt}
\begin{tabular}{ cc }
By Domain & By Year \\  
\input{results-xtables/domain-ns}
& 
\input{results-xtables/Year-ns} \\
\end{tabular}


"Let's turn to the growing concerns over the power of big tech companies." These words came from New York Times national editor Mark Lacey, while moderating a debate among candidates for the 2020 United States presidential election. The candidates were fairly unified on this topic, with responses such as: "we need regulation and reform," "there are absolutely excesses in technology," "they either have to be broken up or regulated," and "I'm not willing to give up and let a handful of monopolists dominate our economy and our democracy."

Algorithmic systems are often the mechanisms through which technology companies can "dominate" some areas of society. For example, consider the company that candidates mentioned most frequently in the debate: Amazon. First and foremost, Amazon's algorithmic systems affect countless transactions whenever users search the platform to buy a product. Also, by algorithmically sifting and sorting through resumes for applicants seeking to work at Amazon, some of the company's algorithmic systems also affect the labor market. Amazon's algorithmic systems also affect public law enforcement, since many agencies use the "Rekognition" facial analysis tool\footnote{\url{https://aws.amazon.com/rekognition}} to analyze security footage.

These growing relationships between algorithms and society have created a need for algorithmic accountability, which can expose problematic behavior in algorithmic systems and give the public an opportunity to respond. For example, in the year leading up to the aforementioned debate, accountability reports exposed problematic behavior in several of Amazon's systems: its product search algorithm was found "to more prominently feature listings that are more profitable for the company" \cite{WSJAmazon2019}, its machine-learning tool used to recommend job candidates was systematically biased against women \cite{ReutersAmazon2018}, and its commercial facial analysis system, "Rekognition," performed worse on female faces and darker-skinned faces \cite{Raji}.


A \textit{discriminatory outcome} is output from an algorithm or algorithmic system which systematically favors or discounts some group(s), leading to disparate impact.

Pearl growing especially helps when researchers use discipline-specific keywords in their writing. For example, empirical studies of "ranking culture" do not use terms such as "algorithmic bias" or "algorithm auditing," but at a high level, they are experimentally equivalent to algorithm audits.

One month prior to the debate, the Wall Street Journal reported that Amazon "adjusted its product-search system to more prominently feature listings that are more profitable for the company."\footnote{\url{https://www.wsj.com/articles/amazon-changed-search-algorithm-in-ways-that-boost-its-own-products-11568645345}} The report illustrated how searches yielded a "proliferation of Amazon's private-label products," which the adjusted algorithm placed mostly on the first page. The public responded, with the company's stock falling in the days after the report.\footnote{\url{https://www.washingtonpost.com/business/on-small-business/amazon-falls-after-report-that-the-company-prioritized-profit-in-its-search-listings/2019/09/16/473162fa-d89d-11e9-a1a5-162b8a9c9ca2_story.html}}

To hold technology companies accountable, it is critical to understand how their algorithmically-driven systems exercise power over the public.


: their systems also have significant power over the information people see (ex. on Google search), political messaging (ex. through Facebook advertising), loan approvals, employment opportunities, everyday navigation, and more. Just as Mark Lacey notes, concerns are "growing" about how technology companies use this power. How can the public hold these systems accountable?

The public responded, and Amazon stock price dropped substantially in the days after the report.\footnote{\url{https://www.washingtonpost.com/business/on-small-business/amazon-falls-after-report-that-the-company-prioritized-profit-in-its-search-listings/2019/09/16/473162fa-d89d-11e9-a1a5-162b8a9c9ca2_story.html}} In short, an algorithmic system was held accountable when work was done to expose problematic behavior.

The candidate suggests that Amazon exercises significant power in society yet lacks meaningful public accountability -- as the baseball analogy illustrates, Amazon simultaneously competes and sets the terms of competition on its platform. 

"Algorithm auditing," a growing area of research in Human-Computer Interaction, shows promise in providing accountability through . For example, 

This kind of work has grown in importance 

How will the public know if a resume ranking algorithm favors male candidates? Or if facial recognition performs better on light-skinned people? Or if text analysis tools associate higher age with lower sentiment? Or if One area of work that seeks to address these questions is the 



\begin{comment}
\subsection{Other Themes}

\subsubsection{Algorithmic Justice and Algorithm Skills}
Eszter Hargittai - who benefits.?

\subsubsection{The Need for an Adversary}

\subsubsection{'Compared to What?'}
Comparative algorithm audits present several benefits over standalone or "single-platform" audits.


\subsubsection{Age}
While several audits of age-related bias appeared during the full-text screening, there is limited work investigating age-related biases in commercial systems. The full-text screening surfaced audits of age-related bias in sentiment analysis \cite{Diaz2018a} and landmark recognition algorithms for facial analysis \cite{Taati2019a}, but no audits of such bias in commercial systems.


\subsubsection{Gender}
Audits of gender bias.


\subsubsection{Skin Type}
The seminal "gender shades" audit examined performance disparities with respect to gender and Fitzpatrick Skin Type, a six-point skin type classification scale used by dermatologists. While the authors identify some problems with the scale (it is skewed toward lighter skin types with "three categories that can be applied to people perceived as White"), they consider it a "scientifically based starting point for auditing algorithms and datasets by skin type."

Audits that look at race and ethnicity.


\subsubsection{Intersectional}
Among the studies reviewed, the "gender shades" study by Buolamwini and Gebru \cite{Buolamwini2018} was the first to discuss \textit{intersectional} biases. Intersectionality identifies how various forms of discrimination occur simultaneously. For example, the error rate for "darker females" was higher than the error rate for "darker" individuals and for "female" individuals. 


\subsubsection{Ideological}
As more researchers scrutinize the effect of algorithmic systems on democracy, a growing body of work is exploring potential ideological bias in these systems. Similar to scholarship that linked bias in other media (ex. television, radio, newspapers) to democratic outcomes,  audits of ideological bias explore the potential for algorithmic systems to affect voting behavior. Many of these audits draw inspiration from the "search engine manipulation effect" (SEME), whereby undecided voters are swayed toward a particular candidate after seeing a search engine results page (SERP). A well-known study shows experimental evidence for this phenomenon, which makes ideological bias a real-world, high-stakes phenomenon to examine through algorithm audits.

Ideological bias has taken on many different definitions and operationalizations...


\subsubsection{Gatekeeping}
Many studies interrogate the ways that algorithms determine which content is made publicly visible. In traditional media studies, this behavior is referred to as "gatekeeping," and some scholars have already used the term "algorithmic gatekeepers" in reference to systems that make such determinations \cite{Napoli2015,Nechushtai2019}.



\subsection{Other Relevant Work}
This literature review focused on accountability audits for algorithms that operate in a public setting. Some audits were found during the screening process that did not meet the eligibility criteria, however, they are relevant to the field of algorithm auditing and noted below.

\subsubsection{User Studies}
Some studies uncovered problematic algorithm behavior through indirect methods such as user surveys and interviews \cite{Fletcher2018b,Eiband2019a,Lee2015Machines}. While these user studies were not included in the review, they provide an effective method for identifying problematic algorithms and painting the "before-and-after picture," as Nissenbaum calls it \cite{Nissenbaum2001}, of the whole socio-technical system. For example, in interviews with Uber and Lyft drivers, \citet{Lee2015Machines} found that algorithmic assignments often did not make sense to the workers, a finding which could help guide an audit study of the assignment algorithms. Díaz and Diakopoulos \cite{Diaz2019b} interview residents about neighborhood walkability, finding that many factors the residents named (ex. places of worship and transit access) were missing in the patented Walk Score algorithm.

\subsubsection{Development History}
Studies that explore the development history of an algorithm can also guide algorithm audits. For example, Gillingham \cite{Gillingham2016} demonstrates a muddled development of predictive tools for child protection services in New Zealand. Devito \cite{DeVito2017} conducts a content analysis of patents, press releases, and other documents to show how values such as personal preferences were considered in Facebook's design of the News Feed algorithm.

\subsubsection{Data Audits}
Studies that audit \textit{data} (such as training data for a machine learning algorithm or the network structure of the world wide web) were not included. Still, researchers may turn to these studies when seeking to explain and understand biases in algorithmic systems.

\subsubsection{Non-commercial Audits}
Due to the focus on public accountability and corporate response, this review did not include several important audits of non-commercial algorithms. Some of these audits found age-related bias in sentiment analysis models \cite{Diaz2018a}, gender bias in semantic representation algorithms that may be used in hiring \cite{De-Arteaga2019}, and age-related disparities in landmark detection algorithms often used for facial analysis \cite{Taati2019a}. Other \cite{Karakasidis2019a}. Other \cite{Binns2017c}.

Text analysis tools such as word embeddings have been shown to exhibit social biases \cite{Caliskan2017,Bolukbasi2016}.


\subsection{Platforms vs. Algorithms vs. Models}


\subsubsection{Some Audits Only Need One Data Point}
Noble \cite{Noble2013} exposes significant problems with just one screenshot of a Google search for "black girls." 

\subsection{Which outcome metrics?}
"partisan bias is a complex, nuanced, and subjective phenomenon that is difficult to quantify in a valid way" \cite{Robertson2018c}.


\subsection{More intersectional audits?}

\subsection{Where does bias come from?}
While Johnson et al. introduced the notion of "structural" algorithmic biases in 2017 \cite{Johnson2017a}, the articles reviewed did not devote significant attention to these biases. While many biases can be attributed to bias in the underlying population or dataset, structural bias is "inherent to the algorithm's design," and cannot be corrected with balanced training data. For example, \cite{Binns2017c} shows that a variety of "toxic comment" classifiers perform worse on female-labelled ground truth, even when those classifiers are trained on female-labelled data.

\end{comment}

==> introduction-old.tex <==
\section{Introduction}
In 2019, Amazon's algorithmic systems 

"Let's turn to the growing concerns over the power of big tech companies." These words came from New York Times national editor Mark Lacey, while moderating a debate among candidates for the 2020 United States presidential election. One candidate responded as follows:
\begin{quote}
Look, I'm not willing to give up and let a handful of monopolists dominate our economy and our democracy... About 49 percent of all sales online happen in one place: that's Amazon... It runs the platform, gets all the information, and then goes into competition with those little businesses. Look, you get to be the umpire in the baseball game, or you get to have a team, but you don't get to do both at the same time.\footnote{\url{https://www.washingtonpost.com/politics/2019/10/15/october-democratic-debate-transcript/}}
\end{quote}

In the months prior to the debate, Amazon's algorithmic systems...

One month prior to the debate, the Wall Street Journal had reported that Amazon "adjusted its product-search system to more prominently feature listings that are more profitable for the company."\footnote{\url{https://www.wsj.com/articles/amazon-changed-search-algorithm-in-ways-that-boost-its-own-products-11568645345}} The report illustrated how searches on Amazon's website yielded a "proliferation" of the company's own private-label products (ex. AmazonBasics), which the tweaked algorithm placed mostly on the first page. As the candidate's baseball analogy suggests, Amazon was simultaneously competing and setting the terms of competition, using their power over a search algorithm in a way that disadvantaged competition.

And yet Amazon product search is just one example of how technology companies have come to "dominate" several areas of our society. To name some salient examples: Google's search algorithm directs attention, Facebook's targeted advertising systems dominate paid political messaging, Uber's pricing algorithm determine wages for a substantial portion of the U.S. labor force, and the YouTube recommendation algorithm drives over 70\% of traffic on the website. As Mark Lacey noted in the debate, this growth in technological power is accompanied with growing concerns about how companies use this power. How will the public hold these systems accountable?

"Algorithm auditing," a growing area of research in Human-Computer Interaction, shows promise in providing accountability through systematic studies of algorithmic systems that may exhibit problematic behavior. In the Amazon example, The Wall Street Journal's report addressed whether Amazon's search algorithm systematically favored its own products. Algorithm auditing can address a wide range of related questions: does Google's search algorithm discount certain news outlets? Does Facebook's targeted advertising system facilitate discrimination? Does Uber's pricing algorithm underpay women? Does the YouTube recommendation algorithm elevate extremist content? With algorithmic systems rapidly growing to affect more people and more areas of society, algorithm audits have become an important way of publicly asking these questions and exposing problematic behavior.

But despite the growing importance and commonality of such work, relatively little effort has gone toward clarifying the past trajectory and future agenda of algorithm auditing. Throughout the history of computing research, growing areas of interest have benefited from systematic literature reviews (SLRs) in early stages, which "identify trends and gaps in the literature" \cite{Dillahunt2017} and help clarify shared research goals for future work. To this end, the present paper conducts an SLR of algorithm audits. It first notes related efforts in existing scholarship, then outlines the method used to identify and review 463 papers, and finally presents results and discussion from a review of 85 papers that met the definition of an algorithm audit.


==> results-domain.tex <==
\section{Results}
This section summarizes review by domain:
\begin{itemize}
\item Internet Search (Section \ref{sec-internet-search})
\item Platform Search (Section \ref{sec-platform-search})
\item Recommender Systems (Section \ref{sec-recommender-systems})
\item Advertising (Section \ref{sec-advertising})
\item Computer Vision (Section \ref{sec-computer-vision})
\item E-Commerce (Section \ref{sec-e-commerce})
\item Criminal Justice (Section \ref{sec-criminal-justice})
\item Language Processing (Section \ref{sec-language-processing})
\end{itemize}


\subsection{Overview}
Based on the studies reviewed, internet search and advertising attracted the most audit attention, and audits appear to be growing in commonality over time:
\begin{center}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{ cc }
By Domain & By Year \\  
\input{results-xtables/domain-ns}
& 
\input{results-xtables/Year-ns} \\
\end{tabular}

\end{center}

\input{results/internet-search}

\input{results/platform-search}

\input{results/recommender-systems}

\input{results/advertising}

\input{results/computer-vision}

\input{results/e-commerce}

\input{results/criminal-justice}

\input{results/language-processing}












==> results-table.tex <==
\begin{longtable}{lllll}
\toprule
                 Reference &  Year &               Domain &                                                           Organization &                                                                      Behavior(s) \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
    \citet{Robertson2019a} &  2019 &      Internet Search &                                              \makecell{Google \\ Bing} &                                       \makecell{Content dependency \\ Stability} \\
    \citet{Robertson2018c} &  2018 &      Internet Search &                                                      \makecell{Google} &                                       \makecell{Partisanship \\ Personalization} \\
                \citet{Hu} &  2019 &      Internet Search &                                                      \makecell{Google} &                                                          \makecell{Partisanship} \\
     \citet{Courtois2018b} &  2018 &      Internet Search &                                                      \makecell{Google} &                                 \makecell{Personalization \\ Content dependency} \\
     \citet{Cano-Oron2019} &  2019 &      Internet Search &                                                      \makecell{Google} &                                       \makecell{Stability \\ Content dependency} \\
           \citet{Trielli} &  2019 &      Internet Search &                                                      \makecell{Google} &                      \makecell{Gatekeeping \\ Content dependency \\ Parisanship} \\
  \citet{Kulshrestha2019b} &  2019 &      Internet Search &                                           \makecell{Google \\ Twitter} &                       \makecell{Content dependency \\ Stability \\ Partisanship} \\
       \citet{Metaxa2019a} &  2019 &      Internet Search &                                                      \makecell{Google} &                                             \makecell{Partisanship \\ Stability} \\
          \citet{Lai2019a} &  2019 &      Internet Search &                                                      \makecell{Google} &                                                       \makecell{Personalization} \\
         \citet{Noble2013} &  2013 &      Internet Search &                                                      \makecell{Google} &                                            \makecell{Racial bias \\ Gender bias} \\
 \citet{Kliman-Silver2015} &  2015 &      Internet Search &                                                      \makecell{Google} &                                                       \makecell{Personalization} \\
        \citet{Hannak2013} &  2013 &      Internet Search &                                                      \makecell{Google} &                                                       \makecell{Personalization} \\
       \citet{Vincent2019} &  2019 &      Internet Search &                                                      \makecell{Google} &                                 \makecell{Content dependency \\ Geographic bias} \\
   \citet{Kulshrestha2017} &  2017 &      Internet Search &                                           \makecell{Twitter \\ Google} &                                                           \makecell{Parisanship} \\
       \citet{McMahon2017} &  2017 &      Internet Search &                                                      \makecell{Google} &                                                    \makecell{Content dependency} \\
               \citet{Kay} &  2015 &      Internet Search &                                                      \makecell{Google} &                                                           \makecell{Gender bias} \\
           \citet{Hannaka} &  2017 &      Platform Search &                                        \makecell{TaskRabbit \\ Fiverr} &  \makecell{Gender bias \\ Racial bias \\ Intersectional bias \\ Geographic bias} \\
           \citet{Moe2019} &  2019 &      Platform Search &                                                     \makecell{YouTube} &                        \makecell{Gatekeeping \\ Stability \\ Content dependency} \\
      \citet{CemGeyik2019} &  2019 &      Platform Search &                                                    \makecell{LinkedIn} &                                                           \makecell{Gender bias} \\
              \citet{Ried} &  2018 &      Platform Search &                                                     \makecell{YouTube} &                        \makecell{Gatekeeping \\ Stability \\ Content dependency} \\
             \citet{Chena} &  2018 &      Platform Search &                          \makecell{Indeed \\ Monster \\ CareerBuilder} &                                                           \makecell{Gender bias} \\
  \citet{Chakraborty2018b} &  2018 &  Recommender Systems &                                              \makecell{New York Times} &                                                       \makecell{Personalization} \\
      \citet{Bechmann2018} &  2018 &  Recommender Systems &                                                    \makecell{Facebook} &                                                       \makecell{Personalization} \\
        \citet{Weber2018a} &  2018 &  Recommender Systems &                                                         \makecell{nan} &                                                           \makecell{Gatekeeping} \\
      \citet{Snickars2017} &  2017 &  Recommender Systems &                                                     \makecell{Spotify} &                                 \makecell{Content dependency \\ Personalization} \\
     \citet{Eriksson2017a} &  2017 &  Recommender Systems &                                                     \makecell{Spotify} &                                                           \makecell{Gender bias} \\
              \citet{Raji} &  2019 &      Computer Vision &                                               \makecell{Amazon; Kairos} &                     \makecell{Gender bias; ;  \\ Skin type \\ Intersectional bias} \\
      \citet{Kyriakou2019} &  2019 &      Computer Vision &  \makecell{Amazon \\ Google \\ IBM \\ Microsoft \\ Imagga \\ Clarifai} &                                            \makecell{Gender bias \\ Racial bias} \\
       \citet{Barlas2019a} &  2019 &      Computer Vision &                                             \makecell{(Same as above)} &                                                       \makecell{(Same as above)} \\
      \citet{DeVries2019a} &  2019 &      Computer Vision &            \makecell{Microsoft \\ Clarifai \\ Google \\ Amazon \\ IBM} &                                                       \makecell{Geographic bias} \\
    \citet{Buolamwini2018} &  2018 &      Computer Vision &                                  \makecell{Microsoft \\ IBM \\ Face++} &                                              \makecell{Skin type \\ Gender bias} \\
    \citet{Lambrecht2019a} &  2019 &          Advertising &          \makecell{Facebook \\ Google AdWords \\ Instagram \\ Twitter} &                                                           \makecell{Gender bias} \\
        \citet{Datta2015a} &  2015 &          Advertising &                                                      \makecell{Google} &                                                      \makecell{Privacy invasion} \\
       \citet{Sweeney2013} &  2013 &          Advertising &                                                      \makecell{Google} &                                                           \makecell{Racial bias} \\
          \citet{Chen2016} &  2016 &           E-commerce &                                                      \makecell{Amazon} &                                                  \makecell{Price discrimination} \\
       \citet{Mikians2012} &  2012 &           E-commerce &                                              \makecell{Google \\ Bing} &                                                       \makecell{Personalization} \\
            \citet{Hannak} &  2014 &           E-commerce &                                \makecell{WalMart \\ Expedia \\ Orbitz} &                                                  \makecell{Price discrimination} \\
      \citet{Matthews2019} &  2019 &     Criminal Justice &                                \makecell{New York City, United States} &                                                     \makecell{Misclassification} \\
             \citet{Tolan} &  2019 &     Criminal Justice &                                            \makecell{Catalonia, Spain} &                          \makecell{Misclassification; Gender bias \\ Racial bias} \\
         \citet{Jiang2019} &  2019 &  Language Processing &                                                     \makecell{YouTube} &                                                          \makecell{Partisanship} \\
\end{longtable}


==> results-tables/advertising.tex <==
\begin{tabular}{lllll}
\toprule
              Reference &  Year &          Audit Type &                                                   Organization &                  Behavior(s) \\
\midrule
    \citet{Sweeney2013} &  2013 &       Direct scrape &                                              \makecell{Google} &       \makecell{Racial bias} \\
     \citet{Datta2015a} &  2015 &  Sock puppet scrape &                                              \makecell{Google} &  \makecell{Privacy invasion} \\
 \citet{Lambrecht2019a} &  2019 &      Carrier puppet &  \makecell{Facebook \\ Google AdWords \\ Instagram \\ Twitter} &       \makecell{Gender bias} \\
\bottomrule
\end{tabular}


==> results-tables/computer-vision.tex <==
\begin{tabular}{lllll}
\toprule
              Reference &  Year &      Audit Type &                                                           Organization &                                                   Behavior(s) \\
\midrule
 \citet{Buolamwini2018} &  2018 &   Direct scrape &                                  \makecell{Microsoft \\ IBM \\ Face++} &                           \makecell{Skin type \\ Gender bias} \\
           \citet{Raji} &  2019 &  Carrier puppet &                                               \makecell{Amazon; Kairos} &  \makecell{Gender bias; ;  \\ Skin type \\ Intersectional bias} \\
   \citet{Kyriakou2019} &  2019 &   Direct scrape &  \makecell{Amazon \\ Google \\ IBM \\ Microsoft \\ Imagga \\ Clarifai} &                         \makecell{Gender bias \\ Racial bias} \\
    \citet{Barlas2019a} &  2019 &   Direct scrape &                                             \makecell{(Same as above)} &                                    \makecell{(Same as above)} \\
   \citet{DeVries2019a} &  2019 &   Direct scrape &            \makecell{Microsoft \\ Clarifai \\ Google \\ Amazon \\ IBM} &                                    \makecell{Geographic bias} \\
\bottomrule
\end{tabular}


==> results-tables/criminal-justice.tex <==
\begin{tabular}{lllll}
\toprule
            Reference &  Year & Audit Type &                             Organization &                                              Behavior(s) \\
\midrule
 \citet{Matthews2019} &  2019 &       Code &  \makecell{New York City, United States} &                             \makecell{Misclassification} \\
        \citet{Tolan} &  2019 &       Code &              \makecell{Catalonia, Spain} &  \makecell{Misclassification; Gender bias \\ Racial bias} \\
\bottomrule
\end{tabular}


==> results-tables/domain-ns.tex <==
\begin{tabular}{lr}
\toprule
              Domain &  Papers Reviewed \\
\midrule
     Internet Search &               16 \\
     Computer Vision &                5 \\
     Platform Search &                5 \\
 Recommender Systems &                5 \\
         Advertising &                3 \\
          E-commerce &                3 \\
    Criminal Justice &                2 \\
 Language Processing &                1 \\
\bottomrule
\end{tabular}


==> results-tables/e-commerce.tex <==
\begin{tabular}{lllll}
\toprule
           Reference &  Year &           Audit Type &                             Organization &                      Behavior(s) \\
\midrule
 \citet{Mikians2012} &  2012 &   Sock puppet scrape &                \makecell{Google \\ Bing} &       \makecell{Personalization} \\
      \citet{Hannak} &  2014 &  Crowdsourced scrape &  \makecell{WalMart \\ Expedia \\ Orbitz} &  \makecell{Price discrimination} \\
    \citet{Chen2016} &  2016 &        Direct scrape &                        \makecell{Amazon} &  \makecell{Price discrimination} \\
\bottomrule
\end{tabular}


==> results-tables/internet-search.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
                 Reference &  Year &           Audit Type &                  Organization &                                                  Behavior(s) \\
\midrule
         \citet{Noble2013} &  2013 &        Direct scrape &             \makecell{Google} &                        \makecell{Racial bias \\ Gender bias} \\
        \citet{Hannak2013} &  2013 &  Crowdsourced scrape &             \makecell{Google} &                                   \makecell{Personalization} \\
 \citet{Kliman-Silver2015} &  2015 &   Sock puppet scrape &             \makecell{Google} &                                   \makecell{Personalization} \\
               \citet{Kay} &  2015 &        Direct scrape &             \makecell{Google} &                                       \makecell{Gender bias} \\
   \citet{Kulshrestha2017} &  2017 &        Direct scrape &  \makecell{Twitter \\ Google} &                                       \makecell{Parisanship} \\
       \citet{McMahon2017} &  2017 &  Crowdsourced scrape &             \makecell{Google} &                                \makecell{Content dependency} \\
    \citet{Robertson2018c} &  2018 &  Crowdsourced scrape &             \makecell{Google} &                   \makecell{Partisanship \\ Personalization} \\
     \citet{Courtois2018b} &  2018 &  Crowdsourced scrape &             \makecell{Google} &             \makecell{Personalization \\ Content dependency} \\
    \citet{Robertson2019a} &  2019 &        Direct scrape &     \makecell{Google \\ Bing} &                   \makecell{Content dependency \\ Stability} \\
                \citet{Hu} &  2019 &        Direct scrape &             \makecell{Google} &                                      \makecell{Partisanship} \\
     \citet{Cano-Oron2019} &  2019 &        Direct scrape &             \makecell{Google} &                   \makecell{Stability \\ Content dependency} \\
           \citet{Trielli} &  2019 &        Direct scrape &             \makecell{Google} &  \makecell{Gatekeeping \\ Content dependency \\ Parisanship} \\
  \citet{Kulshrestha2019b} &  2019 &        Direct scrape &  \makecell{Google \\ Twitter} &   \makecell{Content dependency \\ Stability \\ Partisanship} \\
       \citet{Metaxa2019a} &  2019 &        Direct scrape &             \makecell{Google} &                         \makecell{Partisanship \\ Stability} \\
          \citet{Lai2019a} &  2019 &  Crowdsourced scrape &             \makecell{Google} &                                   \makecell{Personalization} \\
       \citet{Vincent2019} &  2019 &        Direct scrape &             \makecell{Google} &             \makecell{Content dependency \\ Geographic bias} \\
\bottomrule
\end{tabularx}


==> results-tables/language-processing.tex <==
\begin{tabular}{lllll}
\toprule
         Reference &  Year &     Audit Type &        Organization &              Behavior(s) \\
\midrule
 \citet{Jiang2019} &  2019 &  Direct scrape &  \makecell{YouTube} &  \makecell{Partisanship} \\
\bottomrule
\end{tabular}


==> results-tables/platform-search.tex <==
\begin{tabular}{lllll}
\toprule
            Reference &  Year &     Audit Type &                                   Organization &                                                                      Behavior(s) \\
\midrule
      \citet{Hannaka} &  \makecell{2017} &  Direct scrape &                \makecell{TaskRabbit \\ Fiverr} &  \makecell{Gender bias \\ Racial bias \\ Intersectional bias \\ Geographic bias} \\
         \citet{Rieder} &  2018 &  Direct scrape &                             \makecell{YouTube} &                        \makecell{Gatekeeping \\ Stability \\ Content dependency} \\
        \citet{Chena} &  2018 &  Direct scrape &  \makecell{Indeed \\ Monster \\ CareerBuilder} &                                                           \makecell{Gender bias} \\
      \citet{Moe2019} &  2019 &  Direct scrape &                             \makecell{YouTube} &                        \makecell{Gatekeeping \\ Stability \\ Content dependency} \\
 \citet{CemGeyik2019} &  2019 &           Code &                            \makecell{LinkedIn} &                                                           \makecell{Gender bias} \\
\bottomrule
\end{tabular}


==> results-tables/recommender-systems.tex <==
\begin{tabular}{lllll}
\toprule
                Reference &  Year &           Audit Type &               Organization &                                       Behavior(s) \\
\midrule
     \citet{Snickars2017} &  2017 &   Sock puppet scrape &         \makecell{Spotify} &  \makecell{Content dependency \\ Personalization} \\
    \citet{Eriksson2017a} &  2017 &   Sock puppet scrape &         \makecell{Spotify} &                            \makecell{Gender bias} \\
 \citet{Chakraborty2018b} &  2018 &   Sock puppet scrape &  \makecell{New York Times} &                        \makecell{Personalization} \\
     \citet{Bechmann2018} &  2018 &  Crowdsourced scrape &        \makecell{Facebook} &                        \makecell{Personalization} \\
       \citet{Weber2018a} &  2018 &                 Code &             \makecell{nan} &                            \makecell{Gatekeeping} \\
\bottomrule
\end{tabular}


==> results-xtables/Discrimination.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
              Reference &  Year &                                    Method &               Domain &                                                           Organization \\
\midrule
    \citet{Mikians2012} &  2012 &                   \makecell{Sock puppets} &              Pricing &                                              \makecell{Google \\ Bing} \\
   \citet{Mikians2013a} &  2013 &                  \makecell{Crowdsourcing} &              Pricing &                      \makecell{Amazon \\ Hotels.com \\ Other websites} \\
    \citet{Sweeney2013} &  2013 &                  \makecell{Direct scrape} &          Advertising &                                                      \makecell{Google} \\
      \citet{Noble2013} &  2013 &                  \makecell{Direct scrape} &               Search &                                                      \makecell{Google} \\
         \citet{Hannak} &  2014 &  \makecell{Crowdsourcing \\ Sock puppets} &              Pricing &                                \makecell{WalMart \\ Expedia \\ Orbitz} \\
            \citet{Kay} &  2015 &                  \makecell{Direct scrape} &               Search &                                                      \makecell{Google} \\
       \citet{Chen2016} &  2016 &                  \makecell{Direct scrape} &              Pricing &                                                      \makecell{Amazon} \\
  \citet{Eriksson2017a} &  2017 &                   \makecell{Sock puppets} &       Recommendation &                                                     \makecell{Spotify} \\
        \citet{Hannaka} &  2017 &                  \makecell{Direct scrape} &               Search &                                        \makecell{TaskRabbit \\ Fiverr} \\
  \citet{Hupperich2018} &  2018 &                   \makecell{Sock puppets} &              Pricing &                 \makecell{Booking.com \\ Hotels.com \\ Other websites} \\
          \citet{Chena} &  2018 &                  \makecell{Direct scrape} &               Search &                          \makecell{Indeed \\ Monster \\ CareerBuilder} \\
 \citet{Buolamwini2018} &  2018 &                  \makecell{Direct scrape} &               Vision &                                  \makecell{Microsoft \\ IBM \\ Face++} \\
           \citet{Raji} &  2019 &                 \makecell{Carrier puppet} &               Vision &                                            \makecell{Amazon \\ Kairos} \\
    \citet{Barlas2019a} &  2019 &                  \makecell{Direct scrape} &               Vision &                                             \makecell{(Same as below)} \\
   \citet{Kyriakou2019} &  2019 &                  \makecell{Direct scrape} &               Vision &  \makecell{Amazon \\ Google \\ IBM \\ Microsoft \\ Imagga \\ Clarifai} \\
    \citet{DeVries2019} &  2019 &                  \makecell{Direct scrape} &               Vision &            \makecell{Microsoft \\ Clarifai \\ Google \\ Amazon \\ IBM} \\
 \citet{Lambrecht2019a} &  2019 &                 \makecell{Carrier puppet} &          Advertising &          \makecell{Facebook \\ Google AdWords \\ Instagram \\ Twitter} \\
   \citet{CemGeyik2019} &  2019 &                           \makecell{Code} &               Search &                                                    \makecell{LinkedIn} \\
          \citet{Tolan} &  2019 &                           \makecell{Code} &     Criminal Justice &                                            \makecell{Catalonia, Spain} \\
    \citet{Asplund2020} &  2020 &                   \makecell{Sock puppets} &          Advertising &                                                      \makecell{Google} \\
        \citet{Sap2020} &  2020 &                  \makecell{Direct scrape} &  \makecell{Language \\Processing} &                                             \makecell{Jigsaw (Google)} \\
\bottomrule
\end{tabularx}


==> results-xtables/Domain-ns.tex <==
\begin{tabular}{lr}
\toprule
              Domain &  Papers Reviewed \\
\midrule
              Search &               25 \\
         Advertising &               12 \\
      Recommendation &                8 \\
             Pricing &                5 \\
              Vision &                5 \\
    Criminal Justice &                4 \\
 Language Processing &                2 \\
             Mapping &                1 \\
\bottomrule
\end{tabular}


==> results-xtables/Year-ns.tex <==
\begin{tabular}{lr}
\toprule
 Year &  Papers Reviewed \\
\midrule
 2020 &                7 \\
 2019 &               22 \\
 2018 &               14 \\
 2017 &                8 \\
 2016 &                2 \\
 2015 &                3 \\
 2014 &                1 \\
 2013 &                4 \\
 2012 &                1 \\
\bottomrule
\end{tabular}


==> results-xtables/old-tables/Year-ns.tex <==
\begin{tabular}{lr}
\toprule
 Year &  Papers Reviewed \\
\midrule
 2019 &               21 \\
 2018 &               13 \\
 2017 &                7 \\
 2016 &                1 \\
 2015 &                3 \\
 2014 &                1 \\
 2013 &                4 \\
 2012 &                1 \\
\bottomrule
\end{tabular}


==> results-xtables/old-tables/advertising.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
              Reference &  Year &           Audit Type &                          Behavior(s) &                                                                 Organization \\
\midrule
    \citet{Sweeney2013} &  2013 &        Direct scrape &               \makecell{Racial bias} &                                                            \makecell{Google} \\
     \citet{Datta2015a} &  2015 &   Sock puppet scrape &  \makecell{Privacy risks \\ Opacity} &                                                            \makecell{Google} \\
     \citet{Mahler2017} &  2017 &   Direct scrape  &  \makecell{Privacy risks \\ Opacity} &                                                           \makecell{Spotify} \\
    \citet{Cabanas2018} &  2018 &  Crowdsourced scrape &             \makecell{Privacy risks} &                                                          \makecell{Facebook} \\
    \citet{Andreou2018} &  2018 &  Crowdsourced scrape &                   \makecell{Opacity} &                                                          \makecell{Facebook} \\
  \citet{Tschantz2018a} &  2018 &  Crowdsourced scrape &               \makecell{Gender bias} &                                                            \makecell{Google} \\
        \citet{Ali2019} &  2019 &  Crowdsourced scrape  &        \makecell{Exposure diversity} &                                                          \makecell{Facebook} \\
     \citet{Bashir2019} &  2019 &  Crowdsourced scrape &         \makecell{Misclassification} &                                    \makecell{Google \\ Facebook \\ Oracle \\ Neilsen} \\
 \citet{Lambrecht2019a} &  2019 &       Carrier puppet &               \makecell{Gender bias} &                \makecell{Facebook \\ Google AdWords \\ Instagram \\ Twitter} \\
 \citet{Venkatadri2019} &  2019 &  Crowdsourced scrape &         \makecell{Misclassification} &  \makecell{Facebook \\ Acxiom \\ Epsiolon \\ Experian \\ Oracle (Datalogix)} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/computer-vision.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
              Reference &  Year &      Audit Type &                                                   Behavior(s) &                                                           Organization \\
\midrule
 \citet{Buolamwini2018} &  2018 &   Direct scrape &                         \makecell{Racial bias \\ Gender bias} &                                  \makecell{Microsoft \\ IBM \\ Face++} \\
           \citet{Raji} &  2019 &  Carrier puppet &  \makecell{Gender bias \\ Racial bias \\ Intersectional bias} &                                            \makecell{Amazon \\ Kairos} \\
   \citet{Kyriakou2019} &  2019 &   Direct scrape &                         \makecell{Gender bias \\ Racial bias} &  \makecell{Amazon \\ Google \\ IBM \\ Microsoft \\ Imagga \\ Clarifai} \\
    \citet{Barlas2019a} &  2019 &   Direct scrape &                                    \makecell{(Same as above)} &                                             \makecell{(Same as above)} \\
   \citet{DeVries2019} &  2019 &   Direct scrape &                                    \makecell{Geographic bias} &            \makecell{Microsoft \\ Clarifai \\ Google \\ Amazon \\ IBM} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/criminal-justice.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
            Reference &  Year & Audit Type &                                                 Behavior(s) &                 Organization \\
\midrule
     \citet{Duwe2017} &  2017 & Direct scrape  &                                \makecell{Misclassification} &         \makecell{Minnesota} \\
     \citet{Duwe2019} &  2019 & Direct scrape &                                \makecell{Misclassification} &         \makecell{Minnesota} \\
 \citet{Matthews2019} &  2019 &       Code &                                \makecell{Misclassification} &     \makecell{New York City} \\
        \citet{Tolan} &  2019 &       Code &  \makecell{Gender bias \\ Racial bias \\ Misclassification} &  \makecell{Catalonia, Spain} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/domain-ns.tex <==
\begin{tabular}{lr}
\toprule
              Domain &  Papers Reviewed \\
\midrule
     Internet Search &               16 \\
         Advertising &               10 \\
     Computer Vision &                5 \\
          E-commerce &                5 \\
     Platform Search &                5 \\
 Recommender Systems &                5 \\
    Criminal Justice &                4 \\
 Language Processing &                2 \\
\bottomrule
\end{tabular}


==> results-xtables/old-tables/e-commerce.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
             Reference &  Year &           Audit Type &                      Behavior(s) &                                       Organization \\
\midrule
   \citet{Mikians2012} &  2012 &   Sock puppet scrape &  \makecell{Price discrimination} &                          \makecell{Google \\ Bing} \\
  \citet{Mikians2013a} &  2013 &   Crowdsourced scrape &  \makecell{Price discrimination} &        \makecell{Amazon \\ Hotels.com \\ Other websites} \\
        \citet{Hannak} &  2014 &  Crowdsourced scrape &  \makecell{Price discrimination} &            \makecell{WalMart \\ Expedia \\ Orbitz} \\
      \citet{Chen2016} &  2016 &        Direct scrape &  \makecell{Price discrimination} &                                  \makecell{Amazon} \\
 \citet{Hupperich2018} &  2018 &        Crowdsourced scrape  &  \makecell{Price discrimination} &  \makecell{Hotels.com \\ Booking.com \\ Orbitz \\ HRS \\ Avis} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/internet-search.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
                 Reference &  Year &           Audit Type &                                                         Behavior(s) &                  Organization \\
\midrule
         \citet{Noble2013} &  2013 &        Direct scrape &                               \makecell{Racial bias \\ Gender bias} &             \makecell{Google} \\
        \citet{Hannak2013} &  2013 &  Crowdsourced scrape &                                       \makecell{Exposure diversity} &             \makecell{Google} \\
 \citet{Kliman-Silver2015} &  2015 &   Sock puppet scrape &                                       \makecell{Exposure diversity} &             \makecell{Google} \\
               \citet{Kay} &  2015 &        Direct scrape &                                              \makecell{Gender bias} &             \makecell{Google} \\
       \citet{McMahon2017} &  2017 &  Crowdsourced scrape &                                       \makecell{Content dependency} &             \makecell{Google} \\
   \citet{Kulshrestha2017} &  2017 &        Direct scrape &                                              \makecell{Parisanship} &  \makecell{Twitter \\ Google} \\
    \citet{Robertson2018c} &  2018 &  Crowdsourced scrape &                      \makecell{Ideological bias \\ Personalization} &             \makecell{Google} \\
     \citet{Courtois2018b} &  2018 &  Crowdsourced scrape &                 \makecell{Exposure diversity \\ Content dependency} &             \makecell{Google} \\
  \citet{Kulshrestha2019b} &  2018 &        Direct scrape &          \makecell{Content dependency \\ Stability \\ Parisan bias} &  \makecell{Google \\ Twitter} \\
    \citet{Robertson2019a} &  2019 &        Direct scrape &                          \makecell{Content dependency \\ Stability} &     \makecell{Google \\ Bing} \\
                \citet{Hu} &  2019 &        Direct scrape &                                             \makecell{Parisan bias} &             \makecell{Google} \\
     \citet{Cano-Oron2019} &  2019 &        Direct scrape &                          \makecell{Stability \\ Content dependency} &             \makecell{Google} \\
           \citet{Trielli} &  2019 &        Direct scrape &  \makecell{Gatekeeping power \\ Content dependency \\ Parisan bias} &             \makecell{Google} \\
       \citet{Metaxa2019a} &  2019 &        Direct scrape &                                \makecell{Parisan bias \\ Stability} &             \makecell{Google} \\
          \citet{Lai2019a} &  2019 &  Crowdsourced scrape &                                       \makecell{Exposure diversity} &             \makecell{Google} \\
       \citet{Vincent2019} &  2019 &        Direct scrape &                    \makecell{Content dependency \\ Geographic bias} &             \makecell{Google} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/language-processing.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
         Reference &  Year &     Audit Type &               Behavior(s) &                Organization \\
\midrule
 \citet{Jiang2019} &  2019 &  Direct scrape &  \makecell{Partisan bias} &          \makecell{YouTube} \\
   \citet{Sap2020} &  2020 &              &    \makecell{Racial bias} &  \makecell{Jigsaw (Google)} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/platform-search.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
            Reference &  Year &     Audit Type &                                                                      Behavior(s) &                                   Organization \\
\midrule
      \citet{Hannaka} &  2017 &  Direct scrape &  \makecell{Gender bias \\ Racial bias \\ Intersectional bias \\ Geographic bias} &                \makecell{TaskRabbit \\ Fiverr} \\
       \citet{Rieder} &  2018 &  Direct scrape &                 \makecell{Exposure diversity \\ Stability \\ Content dependency} &                             \makecell{YouTube} \\
        \citet{Chena} &  2018 &  Direct scrape &                                                           \makecell{Gender bias} &  \makecell{Indeed \\ Monster \\ CareerBuilder} \\
      \citet{Moe2019} &  2019 &  Direct scrape &                 \makecell{Exposure diversity \\ Stability \\ Content dependency} &                             \makecell{YouTube} \\
 \citet{CemGeyik2019} &  2019 &           Code &                                                           \makecell{Gender bias} &                            \makecell{LinkedIn} \\
\bottomrule
\end{tabularx}


==> results-xtables/old-tables/recommender-systems.tex <==
\begin{tabularx}{\textwidth}{l c X X X}
\toprule
                Reference &  Year &           Audit Type &                                          Behavior(s) &               Organization \\
\midrule
     \citet{Snickars2017} &  2017 &   Sock puppet scrape &  \makecell{Content dependency \\ Exposure diversity} &         \makecell{Spotify} \\
    \citet{Eriksson2017a} &  2017 &   Sock puppet scrape &                               \makecell{Gender bias} &         \makecell{Spotify} \\
 \citet{Chakraborty2018b} &  2018 &   Sock puppet scrape &                        \makecell{Exposure diversity} &  \makecell{New York Times} \\
     \citet{Bechmann2018} &  2018 &  Crowdsourced scrape &                        \makecell{Exposure diversity} &        \makecell{Facebook} \\
       \citet{Weber2018a} &  2018 &                 Code &                        \makecell{Exposure diversity} &             \makecell{} \\
\bottomrule
\end{tabularx}


==> results/advertising.tex <==
\subsection{Advertising}\label{sec-advertising}
While Google makes over 90\% of its revenue from advertising, its advertising systems have received far less audit attention than its search systems. As with the algorithms behind search, algorithms used for targeting, bidding on, and delivering advertisements have a significant effect on the public. The papers reviewed found several types of problematic behavior in advertising systems: \textit{discrimination}, decreased \textit{exposure diversity}, \textit{privacy invasions}, and \textit{misclassification} of users. Table \ref{results-table-advertising} displays all audits reviewed that focused on advertising systems.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/advertising}
}
\caption{Papers reviewed that audit algorithmic advertising systems.}
\label{results-table-advertising}
\end{table}

\subsubsection{Discrimination and Privacy Risks}
One of the first audits of online advertising introduced various ways that ad delivery systems could discriminate toward different groups and individuals. The study, conducted by \citet{Sweeney2013}, shows through case studies and a large-scale analysis of 2,184 name searches that "ads suggesting arrest tend to appear with names associated with blacks, and neutral ads or no ads appear with names associated with whites." \citet{Datta2015a} expanded this evidence to show that protected classes directly affect ad targeting, and later used this evidence to argue that platforms' immunity to Title VII should be reconsidered \cite{Datta2016}.\footnote{In 2019, the U.S. Department of Housing and Urban Development charged Facebook for racial discrimination in targeted housing ads \cite{Paul2019}.}

\citet{Cabanas2018} corroborated these findings, showing that some targeting features explicitly rely on protected and/or sensitive personal attributes such as sexual orientation, political preferences, and religious beliefs. This poses significant privacy risks for users. As a potential way of aligning user expectations of privacy with corporate practice, Facebook added a feature that displays an explanation of why an advertisement appeared. However, an audit revealed that ad explanations are often incomplete and misleading \citep{Andreou2018}.


\subsubsection{Exposure Diversity}
As with search engines, advertising systems have the potential to create "echo chambers" that expose users to a limited set of sources and content. \citet{Ali2019} explored this phenomenon on Facebook's ad delivery system, finding evidence that the system "preferentially exposes users to political advertising." In some cases, even when advertisers with opposing viewpoints targeted users, Facebook preferred to show advertisements that aligned with the users' viewpoints.

\subsubsection{Misclassification}
While advertising systems promise fine-grained targeting, audits show that targeted advertising often does not have accurate information about users. \citet{Tschantz2018a} found that among logged out users across the web, Google correctly inferred age for just 17\% of females and 6\% of males. A 2019 study by \citet{Venkatadri2019} showed a substantial amount of third-party advertisers' data about users is ``not at all accurate'' (40\% of attributes among the 183 users surveyed) -- some users labeled as corporate executives were, in fact, unemployed. Many stakeholders outside academia are interested in the accuracy of targeted advertising \cite{Center}, and further work is needed to clarify how often misclassifications occur.



==> results/computer-vision.tex <==
\subsection{Computer Vision}\label{sec-computer-vision}
Computer vision systems have entered widespread public use, for example, through facial analysis on social networking platforms like Facebook, and object recognition in apps like Google Photos. Many audits of computer vision systems stem from a seminal study by \citet{Buolamwini2018}, which showed that facial analysis on dark-skinned females performed significantly worse than on light-skinned males. The study demonstrated that biases often arise from imbalanced training data, for example, benchmark datsets exhibited "overrepresentation of lighter males, underrepresentation of darker females, and underrepresentation of darker individuals in general" \cite{Buolamwini2018}. Because training data is often imbalanced, and imbalanced data often creates performance disparities, computer vision researchers have since audited a variety of systems for problematic behavior such as \textit{gender bias}, \textit{racial bias}, \textit{geographic bias}, and \textit{intersectional bias}. Table \ref{results-table-computer-vision} displays all audits reviewed that focused on computer vision systems.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/computer-vision}
}
\caption{Papers reviewed that audit public-facing computer vision systems.}
\label{results-table-computer-vision}
\end{table}


\subsubsection{Gender Bias}
Computer vision systems can exhibit gender bias through performance disparities and representation disparities. Performance disparities ocur when a system exhibits higher error rates for a given gender. Similar to findings by \citet{Buolamwini2018}, \citet{Kyriakou2019} found that several commercial systems for image tagging perform worse on female faces. In terms of representation disparities, one of the earliest algorithm audits by \citet{Kay} found that women were consistently underrepresented in Google's image search results compared to metrics from the U.S. Bureau of Labor Statistics.

\subsubsection{Racial Bias}
Racial bias in photographic technology has been present for decades in cinema and photography \cite{Latif2017}, and in some ways, this bias appears to continue with computer vision. In a well-publicized incident involving the Google Photos app, one headline stated "Google Mistakenly Tags Black People as 'Gorillas'"\footnote{\url{https://blogs.wsj.com/digits/2015/07/01/google-mistakenly-tags-black-people-as-gorillas-showing-limits-of-algorithms/}}. While not always as egregious, formal audits of computer vision systems have consistently surfaced similar racial biases: an audit of five commercial image tagging systems \cite{Kyriakou2019,Barlas2019a} found worse performance on people with dark skin, a finding consistent with the original gender shades study \cite{Buolamwini2018} as well as a follow-up study that found performance disparities in three other commercial systems \cite{Raji}.


\subsubsection{Geographic Bias}
Recent work has explored geographic biases in computer vision systems that may arise from skewed training data. In particular, many popular training datasets consist of mostly images from North America and Europe, with fewer images from the global south. As with gender and race, this imbalanced training data results in performance disparities: "object-classification accuracy in recognizing household items is substantially higher for high-income households than it is for low-income households" \cite{DeVries2019a}.


\subsubsection{Intersectional Bias}
The original gender shades study demonstrated the importance of intersectional bias, and the need to account for people belonging to multiple demographic groups. While the three commercial systems exhibited some disparities between male faces and female faces, as well as between darker-skinned and lighter-skinned faces, disparities amplified when they were considered simultaneously. For example, the Face++ error rate among lighter-skiinned males was 0.8\%, while the error rate among darker-skinned females was 34.5\%.


==> results/criminal-justice.tex <==
\subsection{Criminal Justice}\label{sec-criminal-justice}
Computational systems used in criminal justice have been scrutinized since ProPublica's 2016 report entitled "Machine Bias" \cite{Kirchner2016}, which suggested that a publicly-used recidivism prediction instrument (RPI) exhibited racial bias. The report prompted many discussions and explorations of fairness criteria and methods for balancing error rates \cite{Chouldechova2017,Flores2016}. While these theoretical and methodological explorations are not included in this review, only a handful of papers audited computational systems used in criminal justice.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/criminal-justice}
}
\caption{Papers reviewed that audit algorithmic systems used in criminal justice.}
\label{results-table-internet-search}
\end{table}

In a proactive audit of machine learning algorithms that could replace a risk assessment tool called Structured Asssessment of Violence Risk in Youth (SAVRY), \citet{Tolan} warned that the algorithms would discriminate "across sex and national groups across the chosen fairness benchmarks." Two of the studies reviewed \cite{Duwe2017,Duwe2019} focused on recidivism prediction systems in the state of Minnesota, and detailed methods to improving prediction accuracy. Lastly, in a code audit of a forensic DNA analysis system in New York City, \citet{Matthews2019} showed how an allegedly "minor" change to the algorithm resulted in substantial data-dropping that skewed the output toward inaccurate results. The change to removal criteria caused substantial data-dropping that excluded more true contributors and included more non-contributors for the DNA samples analyzed.



==> results/e-commerce.tex <==
\subsection{E-commerce}\label{sec-e-commerce}
E-commerce systems have mostly received attention for dynamic pricing algorithms, which sell the same item to different users at different price points. While dynamic pricing algorithms create the possibility for problems such as predatory pricing and gender-based price discrimination, the audits reviewed focused on the presence of \textit{dynamic pricing}. Table \ref{results-table-e-commerce} displays all audits reviewed that focused on e-commerce systems.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/e-commerce}
}
\caption{Papers reviewed that audit e-commerce systems.}
\label{results-table-e-commerce}
\end{table}


\citet{Mikians2012} presented the first evidence for dynamic pricing in 2012, finding that web history and geographic location affected the price of online products. \citet{Chen2016} scraped Amazon prices for best-selling items, finding over 500 sellers using some form of dynamic algorithmic pricing. They found that these sellers were more often to receive feedback and win the "Buy Box" on the platform. Finally, \citet{Hannak} not only corroborated these findings, but investigated the features that contributed to price discrimination, identifying several online retailers that change prices based on a user's browser, OS, account log-in, click history, and/or purchase history.

==> results/internet-search.tex <==
\subsection{Internet Search}\label{sec-internet-search}
Internet search audits were the most common type among the papers reviewed, many of which cited the "search engine manipulation effect" (SEME) as motivation. The SEME phenomenon involves a search engine shifting voting behavior in accordance with the results presented by the search engine. For example, a large-scale experiment found that 39\% of users "indicated that they would vote for the candidate who was favored by their search rankings" \cite{Epstein2017a}.

SEME suggests that search engines exert some degree of influence over voting behavior and democratic outcomes, which appears to have guided search engine audits toward \textit{ideological bias}. Some audits also examine the \textit{stability} of results over time, the degree of \textit{exposure diversity} in results, and relationships to \textit{content} providers. Table \ref{results-table-internet-search} displays all audits reviewed that focused on internet search.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/internet-search}
}
\caption{Papers reviewed that audit internet search systems.}
\label{results-table-internet-search}
\end{table}

\subsubsection{Ideological Bias}
Experimental evidence for the SEME prompted an urgent question: \textit{are real-world search engine results biased toward certain political candidates?} This question presents many research challenges such as collecting real-world data and operationalizing ideological bias. Details about these challenges are in the discussion, section \ref{discussion}.

Search engine audits have occasionally surfaced evidence for small but statistically significant ideological biases. One of the earliest studies showing such evidence was in case studies by \citet{Diakopoulos}, who found that searches for Republican candidates yielded a higher proportion of negative articles compared to searches for Democratic candidates, and that the overall partisan bias in results was slightly left-leaning. Several studies have replicated this small but significant left-leaning bias on Google, especially in terms of news items \cite{Trielli,Robertson2018c}. However, the result is open to many different interpretations. 

Also, some studies have found conflicting results. For example, while \citet{Robertson2018c} found a slight left-leaning bias in news items, they also found that "Google's ranking algorithm shifted the average lean of SERPs slightly to the right." Also, \citet{Metaxa2019a} observed "virtually no difference" in the distribution of source partisanship between queries for Democrats versus Republicans.

\citet{Hu} audited the "snippet" text that appears below the blue links on search result pages. They found that partisan cues in the snippet text tends to amplify the partisanship of the original webpage, an effect that was consistent across query topics, left- and right-leaning queries, and different types of webpages (social media, news, sports).

\subsubsection{Stability}
The stability of search engine results is of interest to auditors because changes over time may "surface algorithmic changes as well as reflect current events in the offline world" \cite{Metaxa2019a}. Studies have found Google's search results do not exhibit abrupt changes for medical queries \cite{Cano-Oron2019} and political queries \cite{Kulshrestha2019b,Metaxa2019a}. Stability on platform search systems is slightly different, as presented in section \ref{sec-platform-search}.


\subsubsection{Exposure Diversity}
Because search engines personalize results, some scholars have expressed concern over "echo chambers" that may arise when users are not exposed to diverse information \cite{Bozdag2015}. The earliest personalization audit reviewed was by \citet{Hannak2013}  in 2013, which found that on average only 11.7\% of results were personalized, although personalization occured more often in some query categories ("gadgets," "places," and "politics"). A later study by \citet{Kliman-Silver2015} showed that geolocation had the greatest effect on personalized results.

Generally, studies have shown limited evidence for the "echo chambers" that some scholars have feared. A study of 350 Dutch users found no substantial differences due to personalization \cite{Courtois2018b} across 27 socio-political queries. Moving beyond the "blue links," an audit by \citet{Robertson2018c} measured personalization on all different components of a search engine, such as the "people also ask for" box, "tweet cards," and "knowledge components." The full-page audit "found negligible or non-significant differences between the SERPs" of personalized (logged in to Google) and non-personalized (incognito) windows.

However, these findings may be limited to SERPS for socio-political queries. As the earliest personalization audit showed, the degree of personalization varies across query categories \cite{Hannak2013}. A 2019 study in New Zealand by \citet{Lai2019a} focused on how public officials use search engines. Rather than queries for political candidates and topics, the study used queries that public officials "might perform in the course of their everyday work duties," asking 30 participants to rate the relevance of personalized and non-personalized results. Their findings suggest that up to 20\% of relevant results were removed due to personalization.


\subsubsection{Content Dependency}
Besides the ideological bias, personalization, and stability of internet search engines, an important question remains: \textit{what content actually shows up in search results?} The content makeup has implications not only for users, but also for businesses who rely on web traffic.

Almost all studies reviewed present evidence that search engines depend heavily upon user-generated content (UGC) and journalism content. User-generated content from websites like Wikipedia, Twitter, and StackOverflow have been shown to improve click-through rates on Google \cite{McMahon2017}. \citet{Vincent2019} found that Wikipedia appears in over 80\% of results pages for some types of search queries, further demonstrating the value of UGC to search engines. The study also found that the "News Carousel" appeared in the majority popular and trending queries, often in the top three results.

Motivated by studies suggesting search engines heavily depend upon journalism content, \citet{Trielli} conducted a targeted audit of the "Top Stories" carousel on Google's results page, finding a high concentration of sources (the top five sources of impressions per query were CNN, New York Times, The Verge, The Guardian, and Washington Post). The substantial dependence on mainstream media outlets is also evidenced in studies of medical queries \cite{Cano-Oron2019}, political queries in Dutch-speaking regions \cite{Courtois2018b}, and political queries in the United States \cite{Kulshrestha2019b,Robertson2018c}.

==> results/language-processing.tex <==
\subsection{Language Processing}\label{sec-language-processing}
This review identified two audits of public-facing language processing systems: autocomplete and comment moderation. While some studies have identified biases in semantic embedding tools and other language processing systems \cite{Caliskan2017,Binns2017c,Diaz2018a}, those studies did not meet the inclusion criteria. One study\footnote{\citet{Robertson2019a} audited some language processing components of internet search engines, and was classified under the "internet search" domain.} did meet the criteria and was included in the review.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/language-processing}
}
\caption{Papers reviewed that audit public-facing language processing systems.}
\label{results-table-language-processing}
\end{table}

In an audit of comment moderation on YouTube, \citet{Jiang2019} found that extremist comments, comments with false content, and comments posted after a video was fact-checked were more likely to be moderated. By accounting for factors besides ideology, the findings dispel a perception that YouTube's moderation practices were politically biased. It is important to note that YouTube's moderation system involves a hybrid of algorithmic processes, human moderators, and voluntary moderation, so the behavior found in this study cannot be directly attributed to algorithmic behavior. 

==> results/platform-search.tex <==
\subsection{Platform Search}\label{sec-platform-search}
As with internet search engines, platform search engines are integral to many computational systems. Platforms with high volumes of content rely on filtering and ranking systems (namely search engines and recommender systems) to improve user experience. This subsection summarizes platform search audits, and the following subsection summarizes recommender system audits.

Similar to internet search audits, content-focused platforms like YouTube are often audited for \textit{stability}, \textit{content dependency}, and \textit{personalization}. However, people-focused platforms like LinkedIn potentiate additional problematic behavior such as \textit{gender bias}, \textit{racial bias}, and \textit{intersectional bias}. Table \ref{results-table-platform-search} displays all audits reviewed that focused on platform search.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/platform-search}
}
\caption{Papers reviewed that audit platform search systems.}
\label{results-table-platform-search}
\end{table}

\subsubsection{Stability, Content Dependency, and Personalization}
Two studies in the review \cite{Moe2019,Rieder} audited YouTube's search engine through the lens of "ranking cultures," surfacing several noteworthy patterns on the platform. \citet{Moe2019} found that the search algorithm sometimes boosts "content which have attracted minimal attention" to the top of search result pages. This dovetailed with a finding from \citet{Rieder} which found that the search results boosted "niche entrepreneurs" who used highly-specific "YouTube native" vernacular, sometimes to the disadvantage of established mainstream media producers. These two studies also found a high dependency on "newsy" content, and overall stable results over time. The comparative study by \citet{Moe2019} accounted for variation across three languages: Swedish, Danish, and Norwegian. In Islam-related search queries, the authors found that critical videos varied in prominence across languages (ex. less prominent in Swedish, more prominent in Danish).

\subsubsection{Demographic Biases}
Several studies audit demographic biases in searches of people-focused platforms, especially online job boards. This is especially true when considering intersectional attributes rather than singular demographic attributes. An audit of TaskRabbit and Fiverr published in 2017 \cite{Hannaka} found that in TaskRabbit's search algorithm, "the perception of being a White women or a Black man has a significant negative correlation with rank." In an audit of three different job platforms, \citet{Chena} show that males consistently rank higher in results for job queries, controlling for factors such as skill, education level, experience, and more. The finding is robust to measurements of both group fairness and individual fairness.

==> results/recommender-systems.tex <==
\subsection{Recommender Systems}\label{sec-recommender-systems}
Sometimes referred to as "proactive search" systems \cite{Shokouhi2015a}, recommender systems make suggestions to help users easily locate relevant items (news articles, songs, products, etc.) from a large pool of data. Examples of public-facing recommender systems include news recommenders such as Google News, song recommenders such as Spotify radio, and product recommenders such as the "customers also bought" feature on Amazon. In the studies reviewed, public recommender systems were audited for personalization, gender bias, and content dependencies. Table \ref{results-table-internet-search} displays all audits reviewed that focused on recommender systems.

\begin{table}
\rowcolors{1}{white}{gray!15}
\small{
\input{results-xtables/recommender-systems}
}
\caption{Papers reviewed that audited recommender systems.}
\label{results-table-recommender-systems}
\end{table}

\subsubsection{Personalization}
As with internet search engines, recommender systems have the potential to create "echo chambers" by recommending users a narrow, specific set of content. In a typical depiction of the phenomenon, a user reads recommended news articles with a specific viewpoint, forming a feedback loop with the recommender which continually reinforces that viewpoint. But as with internet search, the "echo chamber" phenomenon has failed to materialize in numerous studies examining Google News recommendations \cite{Haim2018,Nechushtai2019} and the Facebook News Feed \cite{Bechmann2018,Bakshy2015}. One study of the New York Times website found evidence for a potential feedback loop on the "Recommendations for You" page. However, the study focused on a single, explicitly-personalized page of the website, and did not examine ideological or topical differences in the content. Lastly, personalization effects were also minimal in an audit of Spotify's radio recommendations -- not even liking all songs or disliking all songs had a significant impact on recommended songs \cite{Snickars2017}. 

\subsubsection{Gender Bias}
In a study of potentially "gendered streams" on Spotify, \citet{Eriksson2017a} found that approximately 8 out of 10 recommended artists were identified as male. Misrepresentation was consistent across different genres as well as the gender of registered users. In other words, while recommendations were similar between registered male and registered female users, these recommendations were consistently skewed toward male artists.

The proactive audit of LinkedIn's search ranking scheme \cite{CemGeyik2019}, included in the previous section, also audited the ranking scheme for top-k recommendations, and found similar success in improving gender representation. 

\subsubsection{Content Dependency}
As with internet search engines and platform search engines, recommender systems depend on a concentrated subset of content. An audit of Spotify's radio recommendations by \citet{Snickars2017} found several repetitive patterns, for example, the initial song was consistently repeated after about 50 tracks.
